NextBestPath: Efficient 3D Mapping of Unseen Environments

This work addresses the problem of active 3D mapping, where an agent must find an efficient trajectory to exhaustively reconstruct a new scene. Previous approaches mainly predict the next best view near the agent's location, which is prone to getting stuck in local areas. Additionally, existing indoor datasets are insufficient due to limited geometric complexity and inaccurate ground truth meshes. To overcome these limitations, we introduce a novel dataset AiMDoom with a map generator for the Doom video game, enabling to better benchmark active 3D mapping in diverse indoor environments. Moreover, we propose a new method we call next-best-path (NBP), which predicts long-term goals rather than focusing solely on short-sighted views. The model jointly predicts accumulated surface coverage gains for long-term goals and obstacle maps, allowing it to efficiently plan optimal paths with a unified model. By leveraging online data collection, data augmentation and curriculum learning, NBP significantly outperforms state-of-the-art methods on both the existing MP3D dataset and our AiMDoom dataset, achieving more efficient mapping in indoor environments of varying complexity.

==> SupplementaryMaterial/dataset.tex <==

\section{Dataset}

\textbf{Dataset construction.} To ensure that each map offers full accessibility for various robotic platforms such as unmanned aerial vehicles (UAVs) and wheeled robots, we configure all doors and windows to remain open during map generation. 
However, we observe that Obsidian does not consistently guarantee accessibility to all areas. To resolve this, we manually edited each scene to ensure the traversability of windows, doors, and hidden passages.

\textbf{Dataset statistic.} To calculate navigation complexity, we sampled location pairs from four environments ranging in difficulty from simple to insane, at rates of 1\%, 0.1\%, 0.05\%, and 0.02\%, constrained by computational resource limitations. Consequently, our data effectively represents a lower bound of navigation complexity. Despite this conservative sampling approach, our dataset remains the most complex one, offering a significant challenge for future research.

Figure~\ref{fig:dataset_full} presents more examples of maps from our dataset, showcasing various levels and diverse scenarios.





==> SupplementaryMaterial/experiments.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/dataset.png}
    \caption{\textbf{More maps from our dataset.} Rows from top to bottom represent increasing scene complexity, categorized into four levels: Simple, Normal, Hard, Insane.}
    \label{fig:dataset_full}
\end{figure}
\section{Experiments}
\input{tables/results_mp3d_details}
\noindent \textbf{Detailed quantitative results.} Table~\ref{tab:doom_test_training_1} and Table.~\ref{tab:doom_test_training_2} show our superior performance on both the AiMDoom training set and the test set. Furthermore, we offer detailed results for each test scene in MP3D, as illustrated in Table~\ref{tab:comparison-mp3d}.

\noindent \textbf{Qualitative results.} 
We provide additional visual comparisons between our method and the state-of-the-art NBV-based method: MACARONS~\citep{guedon2023macarons}, from Figure.~\ref{fig:comparison1}, Figure.~\ref{fig:comparison3} and Figure.\ref{fig:comparison4}. These comparisons demonstrate that our trajectories consistently exhibit superior performance, whether in simple or complex scenarios. Both methods start from the same pose, indicated by a deep blue colour in the visualizations of trajectories.



% Table 1: ExDoom Simple and Normal
\begin{table*}
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
& \multicolumn{4}{c}{\textbf{AiMDoom Simple}} & \multicolumn{4}{c}{\textbf{AiMDoom Normal}} \\
\cmidrule(lr){2-5} \cmidrule(l){6-9}
& \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
& Final Cov. & AUC & Final Cov. & AUC & Final Cov. & AUC & Final Cov. & AUC \\
\midrule
Random Walk & 0.362 & 0.306 & 0.323 & 0.270 & 0.198 & 0.159 & 0.190 & 0.152 \\
 & {\scriptsize ±0.175} & {\scriptsize ±0.156} & {\scriptsize ±0.156} & {\scriptsize ±0.135} & {\scriptsize ±0.125} & {\scriptsize ±0.104} & {\scriptsize ±0.124} & {\scriptsize ±0.103} \\
FBE & 0.770 & 0.628 & 0.760 & 0.605 & 0.564 & 0.423 & 0.565 & 0.415 \\
 & {\scriptsize ±0.163} & {\scriptsize ±0.147} & {\scriptsize ±0.174} & {\scriptsize ±0.171} & {\scriptsize ±0.171} & {\scriptsize ±0.127} & {\scriptsize ±0.139} & {\scriptsize ±0.109} \\
SCONE & 0.597 & 0.482 & 0.577 & 0.483 & 0.421 & 0.315 & 0.412 & 0.313 \\
 & {\scriptsize ±0.177} & {\scriptsize ±0.158} & {\scriptsize ±0.173} & {\scriptsize ±0.138} & {\scriptsize ±0.138} & {\scriptsize ±0.102} & {\scriptsize ±0.114} & {\scriptsize ±0.087} \\
MACARONS & 0.600 & 0.483 & 0.599 & 0.479 & 0.442 & 0.332 & 0.418 & 0.314 \\
 & {\scriptsize ±0.176} & {\scriptsize ±0.145} & {\scriptsize ±0.200} & {\scriptsize ±0.172} & {\scriptsize ±0.135} & {\scriptsize ±0.104} & {\scriptsize ±0.120} & {\scriptsize ±0.088} \\
\textbf{NBP (Ours)} & \textbf{0.870} & \textbf{0.697} & \textbf{0.879} & \textbf{0.692} & \textbf{0.746} & \textbf{0.538} & \textbf{0.734} & \textbf{0.526} \\
 & {\scriptsize {±0.121}} & {\scriptsize {±0.134}} & {\scriptsize {±0.142}} & {\scriptsize {±0.156}} & {\scriptsize {±0.152}} & {\scriptsize {±0.142}} & {\scriptsize {±0.142}} & {\scriptsize {±0.112}} \\
\bottomrule
\end{tabular}
\caption{{Evaluation results on AiMDoom dataset (Simple and Normal)}.}
\label{tab:doom_test_training_1}
\end{table*}

% Table 2: ExDoom Hard and Insane
\begin{table*}[h!]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
& \multicolumn{4}{c}{\textbf{AiMDoom Hard}} & \multicolumn{4}{c}{\textbf{AiMDoom Insane}} \\
\cmidrule(lr){2-5} \cmidrule(l){6-9}
& \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
& Final Cov. & AUC & Final Cov. & AUC & Final Cov. & AUC & Final Cov. & AUC \\
\midrule
Random Walk & 0.121 & 0.086 & 0.124 & 0.088 & 0.070 & 0.048 & 0.074 & 0.050 \\
 & {\scriptsize ±0.081} & {\scriptsize ±0.062} & {\scriptsize ±0.082} & {\scriptsize ±0.060} & {\scriptsize ±0.049} & {\scriptsize ±0.038} & {\scriptsize ±0.048} & {\scriptsize ±0.035} \\
FBE & 0.426 & 0.310 & 0.425 & 0.311 & 0.313 & 0.226 & 0.330 & 0.239 \\
 & {\scriptsize ±0.119} & {\scriptsize ±0.091} & {\scriptsize ±0.114} & {\scriptsize ±0.080} & {\scriptsize ±0.082} & {\scriptsize ±0.066} & {\scriptsize ±0.097} & {\scriptsize ±0.079} \\
SCONE & 0.271 & 0.199 & 0.290 & 0.210 & 0.204 & 0.146 & 0.196 & 0.140 \\
 & {\scriptsize ±0.100} & {\scriptsize ±0.172} & {\scriptsize ±0.093} & {\scriptsize ±0.072} & {\scriptsize ±0.069} & {\scriptsize ±0.052} & {\scriptsize ±0.079} & {\scriptsize ±0.060} \\
MACARONS & 0.316 & 0.202 & 0.302 & 0.218 & 0.201 & 0.143 & 0.192 & 0.139 \\
 & {\scriptsize ±0.106} & {\scriptsize ±0.074} & {\scriptsize ±0.097} & {\scriptsize ±0.070} & {\scriptsize ±0.068} & {\scriptsize ±0.051} & {\scriptsize ±0.078} & {\scriptsize ±0.058} \\
\textbf{NBP (Ours)} & \textbf{0.627} & \textbf{0.430} & \textbf{0.618} & \textbf{0.432} & \textbf{0.486} & \textbf{0.315} & \textbf{0.472} & \textbf{0.312} \\
 & {\scriptsize {±0.144}} & {\scriptsize {±0.111}} & {\scriptsize {±0.153}} & {\scriptsize {±0.115}} & {\scriptsize {±0.106}} & {\scriptsize {±0.047}} & {\scriptsize {±0.095}} & {\scriptsize {±0.073}} \\
\bottomrule
\end{tabular}
\caption{{Evaluation results on AiMDoom dataset (Hard and Insane)}.}
\label{tab:doom_test_training_2}
\end{table*}





% \begin{table}
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{lcccc|cccc|cccc|cccc}
% \toprule
% & \multicolumn{4}{c}{\textbf{ExDoom Simple}} & \multicolumn{4}{c}{\textbf{ExDoom Normal}} & \multicolumn{4}{c}{\textbf{ExDoom Hard}} & \multicolumn{4}{c}{\textbf{ExDoom Insane}} \\[-0.3ex]
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
% & \multicolumn{2}{c}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} & \multicolumn{2}{c}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} & \multicolumn{2}{c}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} & \multicolumn{2}{c}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\[-0.3ex]
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}


% & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{FC}} & \multicolumn{1}{c}{\textbf{AUC}} \\ [-0.3ex]
% \midrule
% \multirow{2}{*}{\minitab[r]{Random Walk}} & 0.362 & 0.306 & 0.323 & 0.270 & 0.198 & 0.159 & 0.190 & 0.152 & 0.121 & 0.086 & 0.124 & 0.088 & 0.070 & 0.048 & 0.074 & 0.050 \\
% & \scriptsize{±0.175} & \scriptsize{±0.156} & \scriptsize{±0.156} & \scriptsize{±0.135} & \scriptsize{±0.125} & \scriptsize{±0.104} & \scriptsize{±0.124} & \scriptsize{±0.103} & \scriptsize{±0.081} & \scriptsize{±0.062} & \scriptsize{±0.082} & \scriptsize{±0.060} & \scriptsize{±0.049} & \scriptsize{±0.038} & \scriptsize{±0.048} & \scriptsize{±0.035} \\[0.5ex]
% \multirow{2}{*}{\minitab[r]{FBE}} & 0.770 & 0.628 & 0.760 & 0.605 & 0.564 & 0.423 & 0.565 & 0.415 & 0.426 & 0.310 & 0.425 & 0.311 & 0.313 & 0.226 & 0.330 & 0.239 \\
% & \scriptsize{±0.163} & \scriptsize{±0.147} & \scriptsize{±0.174} & \scriptsize{±0.171} & \scriptsize{±0.171} & \scriptsize{±0.127} & \scriptsize{±0.139} & \scriptsize{±0.109} & \scriptsize{±0.119} & \scriptsize{±0.091} & \scriptsize{±0.114} & \scriptsize{±0.080} & \scriptsize{±0.082} & \scriptsize{±0.066} & \scriptsize{±0.097} & \scriptsize{±0.079} \\[0.5ex]
% \multirow{2}{*}{\minitab[r]{SCONE}} & 0.597 & 0.482 & 0.577 & 0.483 & 0.421 & 0.315 & 0.412 & 0.313 & 0.271 & 0.199 & 0.290 & 0.210 & 0.204 & 0.146 & 0.196 & 0.140 \\
% & \scriptsize{±0.177} & \scriptsize{±0.158} & \scriptsize{±0.173} & \scriptsize{±0.138} & \scriptsize{±0.138} & \scriptsize{±0.102} & \scriptsize{±0.114} & \scriptsize{±0.087} & \scriptsize{±0.100} & \scriptsize{±0.172} & \scriptsize{±0.093} & \scriptsize{±0.072} & \scriptsize{±0.069} & \scriptsize{±0.052} & \scriptsize{±0.079} & \scriptsize{±0.060} \\[0.5ex]
% \multirow{2}{*}{\minitab[r]{MACARONS}} & 0.600 & 0.483 & 0.599 & 0.479 & 0.442 & 0.332 & 0.418 & 0.314 & 0.316 & 0.202 & 0.302 & 0.218 & 0.201 & 0.143 & 0.192 & 0.139 \\
% & \scriptsize{±0.176} & \scriptsize{±0.145} & \scriptsize{±0.200} & \scriptsize{±0.172} & \scriptsize{±0.135} & \scriptsize{±0.104} & \scriptsize{±0.120} & \scriptsize{±0.088} & \scriptsize{±0.106} & \scriptsize{±0.074} & \scriptsize{±0.097} & \scriptsize{±0.070} & \scriptsize{±0.068} & \scriptsize{±0.051} & \scriptsize{±0.078} & \scriptsize{±0.058} \\

% \multirow{2}{*}{\minitab[r]{\textbf{NBP (Ours)}}} & \textbf{0.870} & \textbf{0.697} & \textbf{0.879} & \textbf{0.692} & \textbf{0.746} & \textbf{0.538} & \textbf{0.734} & \textbf{0.526} & \textbf{0.627} & \textbf{0.430} & \textbf{0.618} & \textbf{0.432} & \textbf{0.486} & \textbf{0.315} & \textbf{0.472} & \textbf{0.312} \\
% & \scriptsize{\textbf{±0.121}} & \scriptsize{\textbf{±0.134}} & \scriptsize{\textbf{±0.142}} & \scriptsize{\textbf{±0.156}} & \scriptsize{\textbf{±0.152}} & \scriptsize{\textbf{±0.142}} & \scriptsize{\textbf{±0.142}} & \scriptsize{\textbf{±0.112}} & \scriptsize{\textbf{±0.144}} & \scriptsize{\textbf{±0.111}} & \scriptsize{\textbf{±0.153}} & \scriptsize{\textbf{±0.115}} & \scriptsize{\textbf{±0.106}} & \scriptsize{\textbf{±0.047}} & \scriptsize{\textbf{±0.095}} & \scriptsize{\textbf{±0.073}} \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{Evaluation results on AiMDoom dataset}. FC refers to the metric of Final Coverage.}
% \label{tab:doom_test_training}
% \end{table}



% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/macarons_3.png}
%         \caption{MACARONS}
%         \label{fig:first_image}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/ours_3.png}
%         \caption{NBP (Ours)}
%         \label{fig:second_image}
%     \end{minipage}
%     \label{fig:both_images}
% \end{figure}


% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/macarons_4.png}
%         \caption{MACARONS}
%         \label{fig:first_image}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/ours_4.png}
%         \caption{NBP (Ours)}
%         \label{fig:second_image}
%     \end{minipage}
%     \label{fig:both_images}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/macarons_8.png}
%         \caption{MACARONS}
%         \label{fig:first_image}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/ours_8.png}
%         \caption{NBP (Ours)}
%         \label{fig:second_image}
%     \end{minipage}
%     \label{fig:both_images}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/macarons_11.png}
%         \caption{MACARONS}
%         \label{fig:first_image}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/ours_11.png}
%         \caption{NBP (Ours)}
%         \label{fig:second_image}
%     \end{minipage}
%     \label{fig:both_images}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/macarons_12.png}
%         \caption{MACARONS}
%         \label{fig:first_image}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Supplementary Material/ours_12.png}
%         \caption{NBP (Ours)}
%         \label{fig:second_image}
%     \end{minipage}
%     \label{fig:both_images}
% \end{figure}

%



\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/macarons_3.png}
        \caption{MACARONS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/ours_3.png}
        \caption{NBP (Ours)}
    \end{subfigure}
    \caption{\textbf{Comparison 1}: In complex and narrow spaces, the NBV (next-best-view) based method can easily get trapped in a local area. Although our method did not manage to reconstruct all areas in this complex scene, it covered most of the areas.}
    \label{fig:comparison1}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/macarons_8.png}
        \caption{MACARONS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/ours_8.png}
        \caption{NBP (Ours)}
    \end{subfigure}
    \caption{\textbf{Comparison 2}: The NBV-based method can easily "assume" that an area has been fully explored, as it focuses solely on local optimal solutions, similar to this sample. In complex indoor environments, it is often necessary to skip some locally optimal poses.}
    \label{fig:comparison3}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/macarons_11.png}
        \caption{MACARONS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/ours_11.png}
        \caption{NBP (Ours)}
    \end{subfigure}
    \caption{\textbf{Comparison 3}: In relatively simple scenes with some obstacles, the NBV exploration can also become trapped in one area.}
    \label{fig:comparison4}
\end{figure}
\clearpage 
As Figure.~\ref{fig:comparison5} and Figure.~\ref{fig:comparison6} illustrated, we also show that in very complex environments, we could only achieve about 65\% coverage. This is because, in complex environments, our method prioritizes the exploration of areas with multiple valuable goals, ignoring places of lesser current value. After the initial exploration is complete, it is likely to explore other regions, overlooking previously encountered areas with higher value. Consequently, developing methods that aim to achieve a global optimum is a promising and valuable direction for future research.


\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/fail_gt1.png}
        \caption{Ground truth mesh}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/fail_1.png}
        \caption{NBP (Ours)}
    \end{subfigure}
    \caption{\textbf{Failure case 1}: Our method initially prioritizes the exploration of high-value areas, inadvertently neglecting regions of secondary importance. Thus, it results in incomplete reconstruction in the initial area of the beginning trajectory.}
    \label{fig:comparison5}
\end{figure}
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/fail_gt2.png}
        \caption{Ground truth mesh}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Supplementary Material/fail_2.png}
        \caption{NBP (Ours)}
    \end{subfigure}
    \caption{\textbf{Failure case 2}: This scene contains multiple narrow areas, prompting our method to depend more heavily on our precise prediction of obstacles. Under these challenging conditions, our approach may overlook exploring this area.}
    \label{fig:comparison6}
\end{figure}



==> SupplementaryMaterial/method.tex <==
\section{Details of mapping process encoder}

We provide more details of the Mapping Process Encoder of our proposed approach in this section.

The mapping encoding is predicted from both the current reconstruction progress and historical trajectory data. At each time step $t \geq 0$, we construct and refine a surface point cloud $\mathcal{P}_t$ by integrating information from newly captured depth map $D_t: \Omega \to \mathbb{R}^+$ and merging it with our existing reconstructed point cloud. For each camera pose $c_t = (c^\text{pos}_t, c^\text{rot}_t)$, we transform the corresponding depth map $D_t$ into a set of 3D points. This transformation makes use of the camera's intrinsic matrix $K \in \mathbb{R}^{3\times3}$ and the pose matrix $T_t \in SE(3)$, derived from the 6D pose $c_t$:
%
\begin{equation}
\mathbf{p}_{surface}(u, v) = T_t \cdot \left( D_t(u, v) \cdot K^{-1} \cdot \begin{bmatrix} u \ v \ 1 \end{bmatrix}^\top \right), \quad (u, v) \in \Omega \> ,
\end{equation}
%
where $\Omega \subset \mathbb{R}^2$ represents the domain of the depth map. We accumulate points over time:
%
\begin{equation}
\mathcal{P}_t = \mathcal{P}_{t-1} \cup \{\mathbf{p}_{surface}(u, v) \mid (u, v) \in \Omega, D_t(u, v) > 0\} \> .
\end{equation}

To enhance scalability and generalization, we introduce a slice mapping approach that transforms the point cloud into a set of $K$ images. We begin by filtering the point cloud based on the camera's position:
%
\begin{equation}
\mathcal{P}_{c_t}^f = \{\mathbf{p} = (p_x, p_y, p_z) \in \mathcal{P}_t \mid |p_x - x_{c_t}| \leq r \text{ and } |p_z - z_{c_t}| \leq r\} \> ,
\end{equation}
%
where $r$ is the radius of our observation window and $(x_{c_t}, y_{c_t}, z_{c_t})$ is the current camera position. We then divide $\mathcal{P}_{c_t}^f$ into $n$ equal vertical slices along the Y-axis, $y_{min}$ and $y_{mmax}$ come from a defined exploration bounding box, as \cite{guedon2023macarons} did:
%
\begin{equation}
\mathcal{S}_{{c_t},j} = \{\mathbf{p} = (p_x, p_y, p_z) \in \mathcal{P}_{c_t}^f \mid y_{min} + (j-1)h_\text{slice} \leq p_y < y_\text{min} + jh_\text{slice}\} \> ,
\end{equation}
%
where $h_\text{slice} = (y_\text{max} - y_\text{min}) / n$ and $j \in {1, \ldots, n}$. Each slice $\mathcal{S}_{{c_t},j}$ is mapped to an image $I_{{c_t},j}$ of size $H \times W$ using a projection function $\phi: \mathbb{R}^3 \to \mathbb{R}^2$:
%
\begin{equation}
\phi(\mathbf{p}) = \left(\left\lfloor\frac{(p_x - x_{c_t} + r) \cdot W}{2r}\right\rfloor, \left\lfloor\frac{(p_z - z_{c_t} + r) \cdot H}{2r}\right\rfloor\right) \> .
\label{projection}
\end{equation}

This projection centres the camera in the middle of the image. Finally, we calculate the point density for each pixel $(u, v)$ in the image $I_{{c_t},j}$:
%
\begin{equation}
I_{{c_t},j}(u, v) = \int_{\mathcal{S}_{{c_t},j}} \delta(\phi(\mathbf{p}) - (u, v)) d\mathbf{p} \> .
\end{equation}
%
Here, $\delta(\cdot)$ is the Dirac delta function and $\mathbf{p}$ represents points from the slice $\mathcal{S}{{c_t},j}$. This process yields $n$ density images ${I_{{c_t},1}, \ldots, I_{{c_t},n}}$ for each time step $t$, effectively transforming 3D point cloud data into 2D representations.

In addition, we apply a similar approach to project the camera's historical trajectory, resulting in a single 2D image. We filter the camera's historical positions based on their proximity to the current camera position in the XZ-plane, using the same threshold $\tau_{xz}$:
%
\begin{equation}
\mathcal{C}_t^f = \{c^{pos}_k = (x_k, y_k, z_k) \mid k < t, |x_k - x_t| \leq \tau_{xz} \text{ and } |z_k - z_t| \leq \tau_{xz}\} \> .
\end{equation}

We then map these filtered positions onto a single image $H_{c_t}$ of the same size $H \times W$:
%
\begin{equation}
H_{c_t}(u, v) = \sum_{c^{pos}_k \in \mathcal{C}_t^f} \delta(\phi(c^{pos}_k) - (u, v))
\end{equation}
%
This results in a single-density image $H_{c_t}$ representing the camera's historical trajectory near its current position. To synthesize the information obtained, we define a set $\mathcal{E}_{c_t}$ encapsulating the entirety of the current exploration embedding: $\mathcal{E}_{c_t} = \{I_{{c_t},1}, \ldots, I_{{c_t},n}, H_{c_t}\}$.



==> arxiv_version/figures/ablation_range.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \vspace{-1em}
    \includegraphics[width=0.5\textwidth]{figures/ablation_range.png}
    \caption{Comparisons of different spatial ranges for value map prediction.}
    \label{fig:ablation_range}
    \vspace{-1em}
\end{wrapfigure}

==> arxiv_version/figures/dataset.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/dataset.png}
%     \caption{\textbf{Top view of samples from our dataset.} Rows from top to bottom represent increasing scene complexity, categorized into four types: \textbf{\textit{Simple, Normal, Hard, Insane}}.}
%     \label{fig:exdoom}
% \end{figure}



\begin{figure}[t]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/doom_top.png}
        \vspace{-1.5em}
        \caption{Bird-eye views of samples from the \textbf{\textit{Simple, Normal, Hard, and Insane}} levels (from left to right).}
        \label{fig:dataset_top}
    \end{subfigure}

    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/doom_inside.png}
        \caption{Representative images showing the internal structural composition of the scene.}
        \label{fig:dataset_inside}
    \end{subfigure}
    \caption{\textbf{Maps from our AiMDoom dataset.} The AiMDoom dataset includes four levels of geometric complexity with various textures.}
    \label{fig:dataset}
    \vspace{-1em}
\end{figure}

==> arxiv_version/figures/pipeline.tex <==
\begin{figure}[t]
    \centering
     \includegraphics[width=\textwidth]{figures/pipeline_iclr_final.png}
    \caption{\textbf{Overview of the proposed next-best-path (NBP) framework.} 
    The model (left, see Section~\ref{sec:method_model}) predicts a value map of coverage gain and an obstacle map, which are used for decision making (right, see Section~\ref{sec:method_decisionmaking}) to obtain a next-best path.
    %Given the current estimate of the surroundings of the agent, we predict the total surface coverage gains after travelling to locations and orientations within a large neighbourhood centered on the agent and an obstacle map for computing the shortest paths towards these locations. See the text for more explanations. 
    }
    \label{fig:pipeline}
    \vspace{-1em}
\end{figure}

==> arxiv_version/figures/teaser.tex <==
\begin{figure}
\centering
\begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/macarons_1.png}
    \caption{MACARONS (simple scene).}
    \label{fig:teaser_macarons}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/ours_1_3.png}
    \caption{Our NBP (simple scene).}
    \label{fig:teaser_ours_1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/ours_2_1.jpg}
    \caption{Our NBP (hard scene).}
    \label{fig:teaser_ours_2}
\end{subfigure}

\caption{
Reconstruction results and trajectories of MACARONS~\citep{guedon2023macarons} and our NBP model. 
\cite{guedon2023macarons} fails to fully map the environment in simple scenes (a), while our NBP model manages to capture the full scene (b), even in much more complex geometry (c).} 
\label{fig:teaser}
\vspace{-1em}
\end{figure}


% \begin{figure}
%     \centering
%     \begin{tabular}{ccc}
%     \adjustbox{valign=c}{\includegraphics[height=2.7cm]{figures/macarons_1.png}} &
%     \adjustbox{valign=c}{\includegraphics[height=2.7cm]{figures/ours_1_3.png}} &
%     \adjustbox{valign=c}{\includegraphics[height=2.7cm]{figures/ours_2_1.jpg}} \\
%     MACARONS trajectory and &
%     Our trajectory and &
%     Our results for a much\\
%     the resulting reconstruction&
%     the resulting reconstruction&
%     more complex scene\\
%     \end{tabular}
%     \caption{\textbf{Left:} Even in relatively simple scenes, state-of-the-art methods~\citep{guedon2023macarons} can fail to fully map the environment, while our NextBestPath method manages to capture the full scene~(\textbf{middle}), even in much more complex geometry (\textbf{right}).} 
%     \label{fig:teaser}
% \end{figure}

==> arxiv_version/figures/training_algorithm.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
\vspace{-1em}
\begin{algorithm}[H]
\caption{Training procedure.}
\label{alg:training}
\begin{algorithmic}
\State $N$: number of training iterations
\State $N_{e}$: number of iterations using easy data
\State $S_n$: the number of trajectories per scene
% \State $P_{c_i}$: Model input
% \State $M_{c_i}^{\text{GT}}[c_g]$: Ground truth heatmap
% \State $O_{c_i}^{\text{GT}}$: Ground truth obstacle map
% \State $n$ = Number of iterations
% \State $m$ = Number of validation samples
% \State $L$ = Trajectory length (100 steps)
\State Initialize memory $\mathcal{M} \leftarrow \emptyset$
\State Initialize model parameter $\theta$
\For{$n \leftarrow 1$ \textbf{to} $N$}
    \State Initialize training set $\mathcal{T} \leftarrow \emptyset$
    \For{each scene in training set}
        \For{$s \leftarrow 1$ \textbf{to} $S_n$}
            \State Collect training data $\{d_l\}_{l=1}^L$
            \If{$n \leq N_e$}
                \State $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l: t \geq 10\}_{l=1}^L$
            \Else
                \State $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l\}_{l=1}^L$
            \EndIf
        \EndFor
    \EndFor
    \State $\mathcal{M} \leftarrow \mathcal{M} \cup \mathcal{T}$
    \State $\mathcal{T} \leftarrow \mathcal{T} \cup \text{RandomSample}(\mathcal{M} \setminus \mathcal{T}, |\mathcal{T}|)$
    % \If{$t > 1$} \Comment{Training starts from the second iteration}
    \For{$e \leftarrow 1$ \textbf{to} $E$}
        \State Update $\theta$ with loss in Eq~\eqref{eqn:training_loss} over $\mathcal{T}$
    \EndFor
\EndFor
\State \Return $\theta$
\end{algorithmic}
\end{algorithm}
\vspace{-3em}
\end{minipage}
\end{wrapfigure}

% \begin{algorithm}
% \caption{Iterative Training Framework with Dynamic Memory and Model-based Data Collection}
% \begin{algorithmic}[1]
% \State $P_{c_i}$: Model input
% \State $M_{c_i}^{\text{GT}}[c_g]$: Ground truth heatmap
% \State $O_{c_i}^{\text{GT}}$: Ground truth obstacle map
% \State $n$ = Number of iterations
% \State $m$ = Number of validation samples
% \State $L$ = Trajectory length (100 steps)
% \State Initialize Memory: $\mathcal{M} = \emptyset$
% \State Initialize Model Parameters: $\theta$
% \For{$t = 1$ \textbf{to} $n$}
%     \State Initialize Training Set: $\mathcal{T} = \emptyset$
%     \For{each scene in training set}
%         \State Collect trajectory: $\{(P_{c_i}, (M_{c_i}^{\text{GT}}[c_g], O_{c_i}^{\text{GT}}))\}_{i=1}^L$ using model
%         \State $\mathcal{T} = \mathcal{T} \cup \{(P_{c_i}, (M_{c_i}^{\text{GT}}[c_g], O_{c_i}^{\text{GT}}))\}_{i=1}^L$
%     \EndFor
%     \State $\mathcal{M} = \mathcal{M} \cup \mathcal{T}$
%     \If{$t = 1$}
%         \State Sample Validation Set: $\mathcal{V} = \text{RandomSample}(\mathcal{M}, m)$
%         \State \textbf{continue} \Comment{Skip training in the first iteration}
%     \ElsIf{$t = 2$}
%         \State Filter $\mathcal{T}$ from $\mathcal{M}$ for $i \geq 10$
%     \Else
%         \State $\mathcal{S} = \text{RandomSample}(\mathcal{M} \setminus \mathcal{T}, |\mathcal{T}|)$
%         \State $\mathcal{T} = \mathcal{T} \cup \mathcal{S}$
%     \EndIf
%     \If{$t > 1$} \Comment{Training starts from the second iteration}
%         \For{$e = 1$ \textbf{to} $5$}
%             \State $\theta = \text{TrainStep}(\theta, \mathcal{T})$ \Comment{Train model to predict $(M_{c_i}^{\text{GT}}[c_g], O_{c_i}^{\text{GT}})$ given $P_{c_i}$}
%         \EndFor
%         \State $\text{val\_loss} = \frac{1}{5} \sum_{e=1}^5 \text{Validate}(\theta, \mathcal{V})$
%         \If{$\text{val\_loss}$ not decreasing}
%             \State \textbf{break}
%         \EndIf
%     \EndIf
% \EndFor
% \State \Return $\theta$
% \end{algorithmic}
% \end{algorithm}


==> arxiv_version/figures/training_algorithm_alt.tex <==
% \begin{algorithm}
% \caption{Training procedure.}
% \label{alg:training}
% \begin{algorithmic}
% \State $N$: number of training iterations, $N_{e}$: number of iterations using easy data
% \State $S_n$: the number of trajectories per scene
% \State Initialize memory $\mathcal{M} \leftarrow \emptyset$ and model parameters $\theta$ randomly
% \For{$n \leftarrow 1$ \textbf{to} $N$}
%     \State Initialize training set $\mathcal{T} \leftarrow \emptyset$
%     \For{each scene in training set}
%         \For{$s \leftarrow 1$ \textbf{to} $S_n$}
%             \State Collect training data $\{d_l\}_{l=1}^L$
%             \State \textbf{if} $n \leq N_e$ \textbf{then} $\mathcal{T} \leftarrow  \mathcal{T} \cup \{d_l: t \geq 10\}_{l=1}^L$ \textbf{else} $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l\}_{l=1}^L$ \textbf{endif}
%             % \If{$n \leq N_e$} \State $\mathcal{T} \leftarrow  \mathcal{T} \cup \{d_l: t \geq 10\}_{l=1}^L$ \Else  \State $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l\}_{l=1}^L$ \EndIf
%         \EndFor
%     \EndFor
%     \State $\mathcal{M} \leftarrow \mathcal{M} \cup \mathcal{T}$
%     \State $\mathcal{T} \leftarrow \mathcal{T} \cup \text{RandomSample}(\mathcal{M} \setminus \mathcal{T}, |\mathcal{T}|)$
%     % \If{$t > 1$} \Comment{Training starts from the second iteration}
%     \For{$e \leftarrow 1$ \textbf{to} $E$}
%         \State Update $\theta$ with loss in Eq.~(\ref{eqn:training_loss}) over $\mathcal{T}$
%     \EndFor
% \EndFor
% \State \Return $\theta$
% \end{algorithmic}
% \end{algorithm}

\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-2em}
\begin{minipage}{0.55\textwidth}
\begin{algorithm}[H]
\caption{Training procedure.}
\label{alg:training}
\begin{algorithmic}
\small
\State $N$: number of training iterations
\State $N_{e}$: number of iterations using easy data
\State $S_n$: the number of trajectories per scene
\State Initialize memory $\mathcal{M} \leftarrow \emptyset$ and model parameters $\theta$
\For{$n \leftarrow 1$ \textbf{to} $N$}
    \State Initialize training set $\mathcal{T} \leftarrow \emptyset$
    \For{each scene in training set}
        \For{$s \leftarrow 1$ \textbf{to} $S_n$}
            \State Collect training data $\{d_l\}_{l=1}^L$
            \State \textbf{if} $n \leq N_e$ \textbf{then} $\mathcal{T} \leftarrow  \mathcal{T} \cup \{d_l: t \geq 10\}_{l=1}^L$ \\ \qquad\qquad~ \textbf{else} $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l\}_{l=1}^L$ \textbf{endif}
        \EndFor
    \EndFor
    \State $\mathcal{M} \leftarrow \mathcal{M} \cup \mathcal{T}$
    \State $\mathcal{T} \leftarrow \mathcal{T} \cup \text{RandomSample}(\mathcal{M} \setminus \mathcal{T}, |\mathcal{T}|)$
    \For{$e \leftarrow 1$ \textbf{to} $E$}
        \State Update $\theta$ with loss in Eq.~(\ref{eqn:training_loss}) over $\mathcal{T}$
    \EndFor
\EndFor
\State \Return $\theta$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-10pt}
\end{wrapfigure}

==> arxiv_version/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arxiv_version/tables/ablation_gt_full.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{Seen} & \multicolumn{2}{c}{Unseen} \\
\multirow{-2}{*}{Method} & Cov. & AUCs & Final Coverage & AUC \\
\midrule
Ours & 0.746 $\pm$ 0.152 & 0.538 $\pm$ 0.142 & 0.734 $\pm$ 0.142 & 0.526 $\pm$ 0.112 \\
Ours (GT-Map) & \textbf{0.817} $\pm$ 0.115 & \textbf{0.586} $\pm$ 0.132 & \textbf{0.808} $\pm$ 0.115 & \textbf{0.580} $\pm$ 0.105 \\
\bottomrule
\end{tabular}
\caption{{Ablation Study on oracle obstacle map.}}
\label{tab:ablation1}
\end{table}

==> arxiv_version/tables/ablation_gt_partial.tex <==
\begin{wraptable}{r}{0.48\textwidth}  % 左对齐，宽度为0.5\textwidth
\caption{{Ablation study on using the oracle map for obstacle avoidance at inference.}}
\centering
\vspace{-0.5em}
\begin{tabular}{lcc}
\toprule
\textbf{Obstacle Map} & \textbf{Final Cov.} & \textbf{AUCs} \\
\midrule
Predicted & 0.734 \tiny{±0.142} & 0.526 \tiny{±0.112} \\
Oracle & \textbf{0.808} \tiny{±0.115} & \textbf{0.580} \tiny{±0.105} \\
\bottomrule
\end{tabular}%
\label{tab:ablation_gt}
\vspace{-1em}
\end{wraptable}

==> arxiv_version/tables/ablation_multi_full.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\
\multirow{-2}{*}{Method} & Cov. & AUCs & Cov. & AUCs \\
\midrule
Ours & 0.714 $\pm$ 0.157 & 0.521 $\pm$ 0.138 & 0.712 $\pm$ 0.136 & 0.501 $\pm$ 0.101 \\
Ours (multi) & \textbf{0.746} $\pm$ 0.152 & \textbf{0.538} $\pm$ 0.142 & \textbf{0.734} $\pm$ 0.142 & \textbf{0.526} $\pm$ 0.112 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on multi-task learning on Normal dataset}}
\label{tab:ablation_multi_full}
\end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{lcc}
\toprule
Method & Cov. & AUCs \\
\midrule
Ours & 0.712 $\pm$ 0.136 & 0.501 $\pm$ 0.101 \\
Ours (multi) & \textbf{0.734} $\pm$ 0.142 & \textbf{0.526} $\pm$ 0.112 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on multi-task learning}}
\label{tab:ablation_multi_unseen}
\end{table}

==> arxiv_version/tables/ablation_multi_partial.tex <==
\begin{wraptable}{l}{0.4\textwidth}  % 左对齐，宽度为0.5\textwidth
\vspace{-0.8em}
\caption{Comparison of single-task and multi-task learning for the value map and obstacle map prediction.}
%
\centering
\tabcolsep=0.07cm

\begin{tabular}{lcc}
\toprule
\textbf{Strategy} & \textbf{Final Cov.} & \textbf{AUCs} \\
\midrule
Single-task & 0.712 \tiny{±0.136} & 0.501 \tiny{±0.101} \\
Multi-task & \textbf{0.734} \tiny{±0.142} & \textbf{0.526} \tiny{±0.112} \\
\bottomrule
\end{tabular}%


\label{tab:ablation_multi_unseen}
\vspace{-1em}
\end{wraptable}

==> arxiv_version/tables/ablation_range.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\
\multirow{-2}{*}{Method} & Cov. & AUCs & Cov. & AUCs \\
\midrule
Ours(big) & 0.713 $\pm$ 0.170 & 0.521 $\pm$ 0.139 & 0.707 $\pm$ 0.140 & 0.517 $\pm$ 0.101 \\
Ours(small) & 0.737 $\pm$ 0.121 & 0.509 $\pm$ 0.135 & 0.729 $\pm$ 0.169 & \textbf{0.529} $\pm$ 0.105 \\
Ours & \textbf{0.746} $\pm$ 0.152 & \textbf{0.538} $\pm$ 0.142 & \textbf{0.734} $\pm$ 0.142 & 0.526 $\pm$ 0.112 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on multi-task learning on Normal dataset}}
\label{tab:ablation1}
\end{table}

==> arxiv_version/tables/dataset_cmpr.tex <==
\begin{table}
\caption{\textbf{Comparison between AiMDoom and prior indoor 3D datasets.} Navigation complexity is the maximum ratio of geodesic to euclidean distances between any two navigable locations in the scene. Universal accessibility means whether windows and doors are accessible.}
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lcccccccccc}
\hline
\noalign{\vskip 1.5mm}
\multicolumn{1}{c}{\multirow{2}{*}{\makecell{Dataset}}} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{Replica}}} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{RoboTHOR}}} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{MP3D}}} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{Gibson\\(4+ only)}}} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{ScanNet}}} & \multicolumn{1}{c}{\multirow{2}{*}{\makecell{HM3D}}} & \multicolumn{4}{c}{\textbf{AiMDoom (Ours)}} \\
\cline{8-11}
\noalign{\vskip 1.1mm}
 &  &  &  &  &  &  & Simple & Normal & Hard & Insane \\
\noalign{\vskip 1mm}
\hline
\noalign{\vskip 1mm}
Number of scenes & 18 & 75 & 90 & 571 (106) & 1613 & 1000 & 100 & 100 & 100 & 100 \\
Floor space (m$^2$) & 2.19k & 3.17k & 101.82k & 217.99k (17.74k) & 39.98k & 365.42k & 63.33k & 134.84k & 321.38k & 548.85k \\
Navigation complexity & 5.99 & 2.06 & 17.09 & 14.25 (11.90) & 3.78 & 13.31 & 11.31 & 18.38 & 36.05 & 45.25 \\
Universal accessibility & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
Easy expansion & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:dataset_comparision}
\vspace{-1em}
\end{table}

==> arxiv_version/tables/results_doom_all.tex <==
\begin{table}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l *{16}{c}}
\toprule
& \multicolumn{4}{c}{\textbf{ExDoom Simple}} & \multicolumn{4}{c}{\textbf{ExDoom Normal}} & \multicolumn{4}{c}{\textbf{ExDoom Hard}} & \multicolumn{4}{c}{\textbf{ExDoom Insane}} \\[-0.3ex]
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
& \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} \\[-0.3ex]
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
& \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} \\[-0.3ex]
& \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & \\[0.5ex]
\midrule
\multirow{2}{*}{\minitab[r]{Random Walk}} & 0.362 & 0.306 & 0.323 & 0.270 & 0.198 & 0.159 & 0.190 & 0.152 & 0.121 & 0.086 & 0.124 & 0.088 & 0.070 & 0.048 & 0.074 & 0.050 \\
& \scriptsize{±0.175} & \scriptsize{±0.156} & \scriptsize{±0.156} & \scriptsize{±0.135} & \scriptsize{±0.125} & \scriptsize{±0.104} & \scriptsize{±0.124} & \scriptsize{±0.103} & \scriptsize{±0.081} & \scriptsize{±0.062} & \scriptsize{±0.082} & \scriptsize{±0.060} & \scriptsize{±0.049} & \scriptsize{±0.038} & \scriptsize{±0.048} & \scriptsize{±0.035} \\[0.5ex]
\multirow{2}{*}{\minitab[r]{FBE}} & 0.770 & 0.628 & 0.760 & 0.605 & 0.564 & 0.423 & 0.565 & 0.415 & 0.426 & 0.310 & 0.425 & 0.311 & 0.313 & 0.226 & 0.330 & 0.239 \\
& \scriptsize{±0.163} & \scriptsize{±0.147} & \scriptsize{±0.174} & \scriptsize{±0.171} & \scriptsize{±0.171} & \scriptsize{±0.127} & \scriptsize{±0.139} & \scriptsize{±0.109} & \scriptsize{±0.119} & \scriptsize{±0.091} & \scriptsize{±0.114} & \scriptsize{±0.080} & \scriptsize{±0.082} & \scriptsize{±0.066} & \scriptsize{±0.097} & \scriptsize{±0.079} \\[0.5ex]
\multirow{2}{*}{\minitab[r]{SCONE}} & 0.597 & 0.482 & 0.577 & 0.483 & 0.421 & 0.315 & 0.412 & 0.313 & 0.271 & 0.199 & 0.290 & 0.210 & 0.204 & 0.146 & 0.196 & 0.140 \\
& \scriptsize{±0.177} & \scriptsize{±0.158} & \scriptsize{±0.173} & \scriptsize{±0.138} & \scriptsize{±0.138} & \scriptsize{±0.102} & \scriptsize{±0.114} & \scriptsize{±0.087} & \scriptsize{±0.100} & \scriptsize{±0.172} & \scriptsize{±0.093} & \scriptsize{±0.072} & \scriptsize{±0.069} & \scriptsize{±0.052} & \scriptsize{±0.079} & \scriptsize{±0.060} \\[0.5ex]
\multirow{2}{*}{\minitab[r]{MACARONS}} & 0.600 & 0.483 & 0.599 & 0.479 & 0.442 & 0.332 & 0.418 & 0.314 & 0.316 & 0.202 & 0.302 & 0.218 & 0.201 & 0.143 & 0.192 & 0.139 \\
& \scriptsize{±0.176} & \scriptsize{±0.145} & \scriptsize{±0.200} & \scriptsize{±0.172} & \scriptsize{±0.135} & \scriptsize{±0.104} & \scriptsize{±0.120} & \scriptsize{±0.088} & \scriptsize{±0.106} & \scriptsize{±0.074} & \scriptsize{±0.097} & \scriptsize{±0.070} & \scriptsize{±0.068} & \scriptsize{±0.051} & \scriptsize{±0.078} & \scriptsize{±0.058} \\

\multirow{2}{*}{\minitab[r]{NBP (Ours)}} & 0.870 & 0.697 & 0.879 & 0.692 & 0.746 & 0.538 & 0.734 & 0.526 & 0.627 & 0.430 & 0.618 & 0.432 & 0.486 & 0.315 & 0.472 & 0.312 \\
& \scriptsize{±0.121} & \scriptsize{±0.134} & \scriptsize{±0.142} & \scriptsize{±0.156} & \scriptsize{±0.152} & \scriptsize{±0.142} & \scriptsize{±0.142} & \scriptsize{±0.112} & \scriptsize{±0.144} & \scriptsize{±0.111} & \scriptsize{±0.153} & \scriptsize{±0.115} & \scriptsize{±0.106} & \scriptsize{±0.047} & \scriptsize{±0.095} & \scriptsize{±0.073} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Evaluation results of baselines and our method on the ExDoom Dataset.} In this table, "Seen" refers to the training dataset, while "Unseen" refers to the test dataset. Considering the varying difficulty levels across the four sub-datasets, we train models respectively for each sub-dataset and for each learning-based method to facilitate a fair comparison.}
\label{tab:doom_main_experiments}
\end{table}

==> arxiv_version/tables/results_mp3d.tex <==
\begin{wraptable}{l}{0.5\textwidth} % This sets the table to the left and defines the width of the wrap area
\centering
\vspace{-0.5em}
\caption{Comparison on the MP3D dataset.}
% \caption{Comparison on the MP3D dataset, the compared methods include: FBE~\cite{fbe}, UPEN~\cite{upen}, OccAnt~\cite{occant}, ANM~\cite{yan2023active}.}
\label{tab:comparison3}
\begin{tabular}{lcc}
\toprule 
\textbf{Method} & \textbf{Comp. (\%) $\uparrow$} & \textbf{Comp. (cm) $\downarrow$} \\
\midrule
Random & 45.67 & 26.53 \\
FBE & 71.18 & 9.78 \\
UPEN & 69.06 & 10.60 \\
OccAnt & 71.72 & 9.40 \\
ANM &  73.15 & 9.11 \\
\textbf{NBP (ours)} & \textbf{79.38} & \textbf{6.78} \\
\bottomrule
\end{tabular}%
\vspace{-0.5em}
\end{wraptable}

==> arxiv_version/tables/results_mp3d_details.tex <==
% \begin{table*}
% \centering
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{lcc|ccccccc|ccccccc}
% & & & \multicolumn{7}{c|}{\textbf{Comp. (\%) $\uparrow$}} & \multicolumn{7}{c}{\textbf{Comp. (cm) $\downarrow$}} \\
% Scene & Rooms & Kfs & Random & FBE & UPEN & OccAnt & ANM & \textbf{NBP (ours)} & & Random & FBE & UPEN & OccAnt & ANM & \textbf{NBP (ours)} & \\
% \toprule 
% GdvgF* & 6 & 32 & 68.45 & 81.78 & 82.39 & 80.24 & 80.99 & \textbf{87.80} & & 11.67 & 5.48 & 5.14 & 5.66 & 5.69 & \textbf{4.92} &  \\
% gZ6f7 & 1 & 48 & 29.81 & 81.01 & 82.96 & 82.02 & 80.68 & \textbf{89.91} & & 46.48 & 7.06 & 6.14 & 6.19 & 7.43 & \textbf{3.31}  & \\
% HxpKQ* & 8 & 32 & 46.93 & 58.71 & 52.70 & 60.50 & 48.34 & \textbf{66.28} & & 19.10 & 11.75 & 14.11 & 11.75 & 15.96 & \textbf{8.12} & \\
% pLe4w & 2 & 52 & 32.92 & 66.09 & 66.76 & 67.13 & \textbf{76.41} & 71.34 & & 30.79 & 12.78 & 11.82 & 11.51 & \textbf{8.03} & 9.53 & \\
% YmJkq & 4 & 68 & 50.26 & 68.32 & 60.47 & 68.70 & 79.35 & \textbf{81.57} & & 24.61 & 11.85 & 15.77 & 11.90 & 8.46 & \textbf{8.01} & \\
% mean & 4 & 46 & 45.67 & 68.53 & 69.09 & 71.72 & 73.15 & \textbf{79.38} & & 26.53 & 9.78 & 10.60 & 9.40 & 9.11 & \textbf{6.78} & \\
% \bottomrule
% \end{tabular}%
% \end{adjustbox}
% \caption{Evaluation results for each test scenes on MP3D}
% \label{tab:comparison-mp3d}
% \end{table*}
\begin{table*}
\centering
\caption{Evaluation results for each test scene on MP3D dataset.}
\begin{adjustbox}{width=\textwidth}
\fontsize{14}{19}\selectfont  % 这里设置字体大小为11pt，行距为13pt
\begin{tabular}{lc|ccccccc|ccccccc}
\toprule
& & \multicolumn{7}{c|}{\textbf{Comp. (\%) $\uparrow$}} & \multicolumn{7}{c}{\textbf{Comp. (cm) $\downarrow$}} \\
Scene & Rooms & Random & FBE & UPEN & OccAnt & ANM & \textbf{NBP (ours)} & & Random & FBE & UPEN & OccAnt & ANM & \textbf{NBP (ours)} & \\
\midrule 
GdvgF* & 6 & 68.45 & 81.78 & 82.39 & 80.24 & 80.99 & \textbf{87.80} & & 11.67 & 5.48 & 5.14 & 5.66 & 5.69 & \textbf{4.92} &  \\
gZ6f7 & 1 & 29.81 & 81.01 & 82.96 & 82.02 & 80.68 & \textbf{89.91} & & 46.48 & 7.06 & 6.14 & 6.19 & 7.43 & \textbf{3.31}  & \\
HxpKQ* & 8 & 46.93 & 58.71 & 52.70 & 60.50 & 48.34 & \textbf{66.28} & & 19.10 & 11.75 & 14.11 & 11.75 & 15.96 & \textbf{8.12} & \\
pLe4w & 2 & 32.92 & 66.09 & 66.76 & 67.13 & \textbf{76.41} & 71.34 & & 30.79 & 12.78 & 11.82 & 11.51 & \textbf{8.03} & 9.53 & \\
YmJkq & 4 & 50.26 & 68.32 & 60.47 & 68.70 & 79.35 & \textbf{81.57} & & 24.61 & 11.85 & 15.77 & 11.90 & 8.46 & \textbf{8.01} & \\
mean & 4 & 45.67 & 71.18 & 69.06 & 71.72 & 73.15 & \textbf{79.38} & & 26.53 & 9.78 & 10.60 & 9.40 & 9.11 & \textbf{6.78} & \\
\bottomrule
\end{tabular}%
\end{adjustbox}

\label{tab:comparison-mp3d}
\end{table*}


==> figures/training_algorithm.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
\vspace{-1em}
\begin{algorithm}[H]
\caption{Training procedure.}
\label{alg:training}
\begin{algorithmic}
\State $N$: number of training iterations
\State $N_{e}$: number of iterations using easy data
\State $S_n$: the number of trajectories per scene
% \State $P_{c_i}$: Model input
% \State $M_{c_i}^{\text{GT}}[c_g]$: Ground truth heatmap
% \State $O_{c_i}^{\text{GT}}$: Ground truth obstacle map
% \State $n$ = Number of iterations
% \State $m$ = Number of validation samples
% \State $L$ = Trajectory length (100 steps)
\State Initialize memory $\mathcal{M} \leftarrow \emptyset$
\State Initialize model parameter $\theta$
\For{$n \leftarrow 1$ \textbf{to} $N$}
    \State Initialize training set $\mathcal{T} \leftarrow \emptyset$
    \For{each scene in training set}
        \For{$s \leftarrow 1$ \textbf{to} $S_n$}
            \State Collect training data $\{d_l\}_{l=1}^L$
            \If{$n \leq N_e$}
                \State $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l: t \geq 10\}_{l=1}^L$
            \Else
                \State $\mathcal{T} \leftarrow \mathcal{T} \cup \{d_l\}_{l=1}^L$
            \EndIf
        \EndFor
    \EndFor
    \State $\mathcal{M} \leftarrow \mathcal{M} \cup \mathcal{T}$
    \State $\mathcal{T} \leftarrow \mathcal{T} \cup \text{RandomSample}(\mathcal{M} \setminus \mathcal{T}, |\mathcal{T}|)$
    % \If{$t > 1$} \Comment{Training starts from the second iteration}
    \For{$e \leftarrow 1$ \textbf{to} $E$}
        \State Update $\theta$ with loss in Eq~\eqref{eqn:training_loss} over $\mathcal{T}$
    \EndFor
\EndFor
\State \Return $\theta$
\end{algorithmic}
\end{algorithm}
\vspace{-3em}
\end{minipage}
\end{wrapfigure}

% \begin{algorithm}
% \caption{Iterative Training Framework with Dynamic Memory and Model-based Data Collection}
% \begin{algorithmic}[1]
% \State $P_{c_i}$: Model input
% \State $M_{c_i}^{\text{GT}}[c_g]$: Ground truth heatmap
% \State $O_{c_i}^{\text{GT}}$: Ground truth obstacle map
% \State $n$ = Number of iterations
% \State $m$ = Number of validation samples
% \State $L$ = Trajectory length (100 steps)
% \State Initialize Memory: $\mathcal{M} = \emptyset$
% \State Initialize Model Parameters: $\theta$
% \For{$t = 1$ \textbf{to} $n$}
%     \State Initialize Training Set: $\mathcal{T} = \emptyset$
%     \For{each scene in training set}
%         \State Collect trajectory: $\{(P_{c_i}, (M_{c_i}^{\text{GT}}[c_g], O_{c_i}^{\text{GT}}))\}_{i=1}^L$ using model
%         \State $\mathcal{T} = \mathcal{T} \cup \{(P_{c_i}, (M_{c_i}^{\text{GT}}[c_g], O_{c_i}^{\text{GT}}))\}_{i=1}^L$
%     \EndFor
%     \State $\mathcal{M} = \mathcal{M} \cup \mathcal{T}$
%     \If{$t = 1$}
%         \State Sample Validation Set: $\mathcal{V} = \text{RandomSample}(\mathcal{M}, m)$
%         \State \textbf{continue} \Comment{Skip training in the first iteration}
%     \ElsIf{$t = 2$}
%         \State Filter $\mathcal{T}$ from $\mathcal{M}$ for $i \geq 10$
%     \Else
%         \State $\mathcal{S} = \text{RandomSample}(\mathcal{M} \setminus \mathcal{T}, |\mathcal{T}|)$
%         \State $\mathcal{T} = \mathcal{T} \cup \mathcal{S}$
%     \EndIf
%     \If{$t > 1$} \Comment{Training starts from the second iteration}
%         \For{$e = 1$ \textbf{to} $5$}
%             \State $\theta = \text{TrainStep}(\theta, \mathcal{T})$ \Comment{Train model to predict $(M_{c_i}^{\text{GT}}[c_g], O_{c_i}^{\text{GT}})$ given $P_{c_i}$}
%         \EndFor
%         \State $\text{val\_loss} = \frac{1}{5} \sum_{e=1}^5 \text{Validate}(\theta, \mathcal{V})$
%         \If{$\text{val\_loss}$ not decreasing}
%             \State \textbf{break}
%         \EndIf
%     \EndIf
% \EndFor
% \State \Return $\theta$
% \end{algorithmic}
% \end{algorithm}


==> figures/viz_results.tex <==
% \begin{figure}
%     \centering
%     \begin{tabular}{c@{\hspace{-0.3cm}}c@{\hspace{0.0cm}}c}
%     \includegraphics[height=3.3cm]{figures/macarons_13.png} &
%     \includegraphics[height=3.3cm]{figures/macarons_9.png} &
%     \includegraphics[height=3.3cm]{figures/macarons_14.png} \\
%     \end{tabular}
%     \vspace{-0.2cm}  
%     \\
%     \subcaption{MACARONS}
%     \begin{tabular}{c@{\hspace{-0.3cm}}c@{\hspace{0.0cm}}c}
%     \includegraphics[height=3.3cm]{figures/ours_13.png} &
%     \includegraphics[height=3.3cm]{figures/ours_9.png} &
%     \includegraphics[height=3.3cm]{figures/ours_14.png} \\
%     \end{tabular}
%     \vspace{-0.2cm}
%     \\
%     \subcaption{NBP (Ours)}
%     \caption{\textbf{Comparison of our method with the state-of-the-art MACARONS method on AiMDoom Simple dataset.} \textbf{MACARONS~(top row)} generates complicated trajectories that do not manage to map the scenes completely even at a simple level. \textbf{Our method (bottom row)} generates efficient trajectories that capture the entire scenes. In the same scenes, both methods start from the same pose, marked in deep blue.}
%     \label{fig:combined_results}
% \end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \begin{tabular}{c@{\hspace{-0.3cm}}c@{\hspace{0.0cm}}c}
        \includegraphics[height=3.3cm]{figures/macarons_13.png} &
        \includegraphics[height=3.3cm]{figures/macarons_9.png} &
        \includegraphics[height=3.3cm]{figures/macarons_14.png} \\
        \end{tabular}
        \vspace{-0.2cm}
        \caption{Results of MACARONS. It generates complicated trajectories and often gets trapped in local areas.}
    \end{subfigure}
    \vspace{0.2cm}  % Adjust this value to control vertical spacing between subfigures
    \begin{subfigure}{\textwidth}
        \centering
        \begin{tabular}{c@{\hspace{-0.3cm}}c@{\hspace{0.0cm}}c}
        \includegraphics[height=3.3cm]{figures/ours_13.png} &
        \includegraphics[height=3.3cm]{figures/ours_9.png} &
        \includegraphics[height=3.3cm]{figures/ours_14.png} \\
        \end{tabular}
        \vspace{-0.2cm}
        \caption{Results of our NBP method. It efficiently travels in the scene and reconstructs the scene well.}
    \end{subfigure}
    \caption{\textbf{Comparison of our NBP method with the state-of-the-art MACARONS method.} Both methods start from the same initial pose, marked in deep blue. {\color{blue}We also include a demonstration video of active mapping using our method in the supplementary materials.}
    % \textbf{MACARONS~(top row)} generates complicated trajectories that do not manage to map the scenes completely even at a simple level. 
    % \textbf{Our method (bottom row)} generates efficient trajectories that capture the entire scenes. In the same scenes, both methods start from the same pose, marked in deep blue.
    }
    \label{fig:combined_results}
    \vspace{-2em}
\end{figure}




==> tables/ablation_gt_full.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{Seen} & \multicolumn{2}{c}{Unseen} \\
\multirow{-2}{*}{Method} & Cov. & AUCs & Final Coverage & AUC \\
\midrule
Ours & 0.746 $\pm$ 0.152 & 0.538 $\pm$ 0.142 & 0.734 $\pm$ 0.142 & 0.526 $\pm$ 0.112 \\
Ours (GT-Map) & \textbf{0.817} $\pm$ 0.115 & \textbf{0.586} $\pm$ 0.132 & \textbf{0.808} $\pm$ 0.115 & \textbf{0.580} $\pm$ 0.105 \\
\bottomrule
\end{tabular}
\caption{{Ablation Study on oracle obstacle map.}}
\label{tab:ablation1}
\end{table}

==> tables/ablation_multi_full.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\
\multirow{-2}{*}{Method} & Cov. & AUCs & Cov. & AUCs \\
\midrule
Ours & 0.714 $\pm$ 0.157 & 0.521 $\pm$ 0.138 & 0.712 $\pm$ 0.136 & 0.501 $\pm$ 0.101 \\
Ours (multi) & \textbf{0.746} $\pm$ 0.152 & \textbf{0.538} $\pm$ 0.142 & \textbf{0.734} $\pm$ 0.142 & \textbf{0.526} $\pm$ 0.112 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on multi-task learning on Normal dataset}}
\label{tab:ablation_multi_full}
\end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{lcc}
\toprule
Method & Cov. & AUCs \\
\midrule
Ours & 0.712 $\pm$ 0.136 & 0.501 $\pm$ 0.101 \\
Ours (multi) & \textbf{0.734} $\pm$ 0.142 & \textbf{0.526} $\pm$ 0.112 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on multi-task learning}}
\label{tab:ablation_multi_unseen}
\end{table}

==> tables/ablation_range.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\
\multirow{-2}{*}{Method} & Cov. & AUCs & Cov. & AUCs \\
\midrule
Ours(big) & 0.713 $\pm$ 0.170 & 0.521 $\pm$ 0.139 & 0.707 $\pm$ 0.140 & 0.517 $\pm$ 0.101 \\
Ours(small) & 0.737 $\pm$ 0.121 & 0.509 $\pm$ 0.135 & 0.729 $\pm$ 0.169 & \textbf{0.529} $\pm$ 0.105 \\
Ours & \textbf{0.746} $\pm$ 0.152 & \textbf{0.538} $\pm$ 0.142 & \textbf{0.734} $\pm$ 0.142 & 0.526 $\pm$ 0.112 \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on multi-task learning on Normal dataset}}
\label{tab:ablation1}
\end{table}

==> tables/results_doom.tex <==
\begin{table}
\caption{\textbf{Evaluation results on AiMDoom Dataset.} 
% Separate models are trained from scratch for each level. 
{\color{blue} For each difficulty level, all baseline models, including ours, are trained from scratch on the corresponding training set to ensure a fair comparison.}
%Considering the varying difficulty levels across the four sub-datasets, we train models respectively for each sub-dataset and for each learning-based method to facilitate a fair comparison.
}
\centering
\footnotesize  % 将整个表格的字体缩小到 \scriptsize
% \renewcommand{\arraystretch}{1.1}  % 稍微减小行距
% \setlength{\tabcolsep}{2pt}  % 进一步减小列间距
\tabcolsep=0.07cm
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l*{8}{c}}
\toprule
& \multicolumn{2}{c}{\textbf{Simple}} & \multicolumn{2}{c}{\textbf{Normal}} & \multicolumn{2}{c}{\textbf{Hard}} & \multicolumn{2}{c}{\textbf{Insane}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& Final Cov. & AUCs & Final Cov. & AUCs & Final Cov. & AUCs & Final Cov. & AUCs \\
\midrule
Random & 0.323\tiny{±0.156} & 0.270\tiny{±0.135} & 0.190\tiny{±0.124} & 0.152\tiny{±0.103} & 0.124\tiny{±0.082} & 0.088\tiny{±0.060} & 0.074\tiny{±0.048} & 0.050\tiny{±0.035} \\
FBE & 0.760\tiny{±0.174} & 0.605\tiny{±0.171} & 0.565\tiny{±0.139} & 0.415\tiny{±0.109} & 0.425\tiny{±0.114} & 0.311\tiny{±0.080} & 0.330\tiny{±0.097} & 0.239\tiny{±0.079} \\
SCONE & 0.577\tiny{±0.173} & 0.483\tiny{±0.138} & 0.412\tiny{±0.114} & 0.313\tiny{±0.087} & 0.290\tiny{±0.093} & 0.210\tiny{±0.072} & 0.196\tiny{±0.079} & 0.140\tiny{±0.060} \\
MACARONS & 0.599\tiny{±0.200} & 0.479\tiny{±0.172} & 0.418\tiny{±0.120} & 0.314\tiny{±0.088} & 0.302\tiny{±0.097} & 0.218\tiny{±0.070} & 0.192\tiny{±0.078} & 0.139\tiny{±0.058} \\
 \textbf{NBP (Ours)} & \textbf{0.879}\tiny{±0.142} & \textbf{0.692}\tiny{±0.156} & \textbf{0.734}\tiny{±0.142} & \textbf{0.526}\tiny{±0.112} & \textbf{0.618}\tiny{±0.153} & \textbf{0.432}\tiny{±0.115} & \textbf{0.472}\tiny{±0.095} & \textbf{0.312}\tiny{±0.073} \\
\bottomrule
\end{tabular*}
\label{tab:doom_main_experiments}
\vspace{-1em}
\end{table}

==> tables/results_doom_all.tex <==
\begin{table}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l *{16}{c}}
\toprule
& \multicolumn{4}{c}{\textbf{ExDoom Simple}} & \multicolumn{4}{c}{\textbf{ExDoom Normal}} & \multicolumn{4}{c}{\textbf{ExDoom Hard}} & \multicolumn{4}{c}{\textbf{ExDoom Insane}} \\[-0.3ex]
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
& \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} \\[-0.3ex]
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
& \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} & \multicolumn{1}{c}{Final} & \multicolumn{1}{c}{\multirow{2}{*}{AUC}} \\[-0.3ex]
& \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & & \multicolumn{1}{c}{Coverage} & \\[0.5ex]
\midrule
\multirow{2}{*}{\minitab[r]{Random Walk}} & 0.362 & 0.306 & 0.323 & 0.270 & 0.198 & 0.159 & 0.190 & 0.152 & 0.121 & 0.086 & 0.124 & 0.088 & 0.070 & 0.048 & 0.074 & 0.050 \\
& \scriptsize{±0.175} & \scriptsize{±0.156} & \scriptsize{±0.156} & \scriptsize{±0.135} & \scriptsize{±0.125} & \scriptsize{±0.104} & \scriptsize{±0.124} & \scriptsize{±0.103} & \scriptsize{±0.081} & \scriptsize{±0.062} & \scriptsize{±0.082} & \scriptsize{±0.060} & \scriptsize{±0.049} & \scriptsize{±0.038} & \scriptsize{±0.048} & \scriptsize{±0.035} \\[0.5ex]
\multirow{2}{*}{\minitab[r]{FBE}} & 0.770 & 0.628 & 0.760 & 0.605 & 0.564 & 0.423 & 0.565 & 0.415 & 0.426 & 0.310 & 0.425 & 0.311 & 0.313 & 0.226 & 0.330 & 0.239 \\
& \scriptsize{±0.163} & \scriptsize{±0.147} & \scriptsize{±0.174} & \scriptsize{±0.171} & \scriptsize{±0.171} & \scriptsize{±0.127} & \scriptsize{±0.139} & \scriptsize{±0.109} & \scriptsize{±0.119} & \scriptsize{±0.091} & \scriptsize{±0.114} & \scriptsize{±0.080} & \scriptsize{±0.082} & \scriptsize{±0.066} & \scriptsize{±0.097} & \scriptsize{±0.079} \\[0.5ex]
\multirow{2}{*}{\minitab[r]{SCONE}} & 0.597 & 0.482 & 0.577 & 0.483 & 0.421 & 0.315 & 0.412 & 0.313 & 0.271 & 0.199 & 0.290 & 0.210 & 0.204 & 0.146 & 0.196 & 0.140 \\
& \scriptsize{±0.177} & \scriptsize{±0.158} & \scriptsize{±0.173} & \scriptsize{±0.138} & \scriptsize{±0.138} & \scriptsize{±0.102} & \scriptsize{±0.114} & \scriptsize{±0.087} & \scriptsize{±0.100} & \scriptsize{±0.172} & \scriptsize{±0.093} & \scriptsize{±0.072} & \scriptsize{±0.069} & \scriptsize{±0.052} & \scriptsize{±0.079} & \scriptsize{±0.060} \\[0.5ex]
\multirow{2}{*}{\minitab[r]{MACARONS}} & 0.600 & 0.483 & 0.599 & 0.479 & 0.442 & 0.332 & 0.418 & 0.314 & 0.316 & 0.202 & 0.302 & 0.218 & 0.201 & 0.143 & 0.192 & 0.139 \\
& \scriptsize{±0.176} & \scriptsize{±0.145} & \scriptsize{±0.200} & \scriptsize{±0.172} & \scriptsize{±0.135} & \scriptsize{±0.104} & \scriptsize{±0.120} & \scriptsize{±0.088} & \scriptsize{±0.106} & \scriptsize{±0.074} & \scriptsize{±0.097} & \scriptsize{±0.070} & \scriptsize{±0.068} & \scriptsize{±0.051} & \scriptsize{±0.078} & \scriptsize{±0.058} \\

\multirow{2}{*}{\minitab[r]{NBP (Ours)}} & 0.870 & 0.697 & 0.879 & 0.692 & 0.746 & 0.538 & 0.734 & 0.526 & 0.627 & 0.430 & 0.618 & 0.432 & 0.486 & 0.315 & 0.472 & 0.312 \\
& \scriptsize{±0.121} & \scriptsize{±0.134} & \scriptsize{±0.142} & \scriptsize{±0.156} & \scriptsize{±0.152} & \scriptsize{±0.142} & \scriptsize{±0.142} & \scriptsize{±0.112} & \scriptsize{±0.144} & \scriptsize{±0.111} & \scriptsize{±0.153} & \scriptsize{±0.115} & \scriptsize{±0.106} & \scriptsize{±0.047} & \scriptsize{±0.095} & \scriptsize{±0.073} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Evaluation results of baselines and our method on the ExDoom Dataset.} In this table, "Seen" refers to the training dataset, while "Unseen" refers to the test dataset. Considering the varying difficulty levels across the four sub-datasets, we train models respectively for each sub-dataset and for each learning-based method to facilitate a fair comparison.}
\label{tab:doom_main_experiments}
\end{table}
